Towards AIOps in Edge Computing Environments

Edge computing was introduced as a technical enabler for the demanding requirements of new network technologies like 5G. It aims to overcome challenges related to centralized cloud computing environments by distributing computational resources to the edge of the network towards the customers. The complexity of the emerging infrastructures increases significantly, together with the ramifications of outages on critical use cases such as self-driving cars or health care. Artificial Intelligence for IT Operations (AIOps) aims to support human operators in managing complex infrastructures by using machine learning methods. This paper describes the system design of an AIOps platform which is applicable in heterogeneous, distributed environments. The overhead of a high-frequency monitoring solution on edge devices is evaluated and performance experiments regarding the applicability of three anomaly detection algorithms on edge devices are conducted. The results show, that it is feasible to collect metrics with a high frequency and simultaneously run specific anomaly detection algorithms directly on edge devices with a reasonable overhead on the resource utilization.

==> 04-testbed.tex <==
\section{Performance experiments}
Edge devices are typically restricted in terms of processing power, memory and energy consumption (TODO:ref). Since our components were previously only tested
on cloud environments consisting of commodity servers we have run multiple experiments to evaluate the performance and overhead of the collector component and used 
anomaly detection algorithms on edge devices. 


\subsection{Collector Overhead}
We evaluated the overhead of the collector with different frequencies while running on edge devices ( Raspberry Pi 3B and 4).
The results depicted in Figure \textbf{TODO} show, that even with a frequency of 500ms the
overhead of the collector amounts to only \textbf{TODO}.

\missingfigure[figwidth=0.45\textwidth]{Plot CPU overhead of bitflow-collector running on different Raspberry Pis with collecting rates 500ms to 10s for each CPU architecture}
\begin{tikzpicture}
            \begin{axis}[
                xlabel={Frequency in ms},
                ylabel={CPU usage},
                xmin=100, xmax=10000,
                ymin=0, %ymax=1400,
                %xtick={0,1,2,3,4},
                %ytick={0,200,400,600,800,1000,1200,1400, 1600. 1800, 2000, 2200, 2400 },
                legend pos=north east,
                ymajorgrids=true,
                grid style=dashed,
            ]
            \addplot table[x=cpu,y expr=\thisrow{CABIRCH} * 0.001 ,col sep=comma] {results/results_average_wally025.csv}; \addlegendentry{CABIRCH}
            \end{axis}
        \end{tikzpicture}


\subsection{Performace of Anomaly Detection Algorithms}
The ARIMA, CABIRCH, and LSTM anomaly detection algorithms were implemented in Java and integrated into the Bitflow framework.
We are using Docker as execution platform which allows us to limit the resources of running processes and performed the following experiment on
a commodity server, a Raspberry Pi 4 with arm64v8 CPU architecture and a Raspberry Pi 3B with with arm32v7 architecture:

In each experiment run, a data set of 10.000 samples with 28 metrics in each sample was processed by the respective algorithm,
while measuring the average processing time per sample, and the standard deviation. In case of the commodity server, we started with no resource limitation at all
(8 virtual CPUs) and decreased the allocated vCPUs by 0.1 for each following run until reaching the reaching the minimum assignable
resources at 0.1 CPUs. For the Rasperry Pis we compiled a custom Raspbian Linux kernel since the default kernel doesn't support the \textit{cpu.cfs\_period\_us} and 
\textit{cpu.cfs\_quota\_us} cgroups used by the Docker engine for the resource limitation.
Afterwards we ran the same experiments on those devices starting with 4 vCPUs.

Figure \ref{aa_experiments} shows the results of the evaluation
\todo{run all experiments and compare}



\begin{figure*}[]
    \centering
    \subcaptionbox{Raspberry Pi (arm32v7)}
        {
        \begin{tikzpicture}
            \begin{axis}[
                xlabel={CPUs},
                ylabel={s/sample},
                xmin=0, xmax=4,
                ymin=0, %ymax=1400,
                xtick={0,1,2,3,4},
                %ytick={0,200,400,600,800,1000,1200,1400, 1600. 1800, 2000, 2200, 2400 },
                legend pos=north east,
                ymajorgrids=true,
                grid style=dashed,
            ]
            \addplot table[x=cpu,y expr=\thisrow{CABIRCH} * 0.001 ,col sep=comma] {results/rpi4.csv}; \addlegendentry{CABIRCH}
            \addplot table[x=cpu,y expr=\thisrow{LSTM} * 0.001 ,col sep=comma] {results/rpi4.csv}; \addlegendentry{LSTM}
            \addplot table[x=cpu,y expr=\thisrow{ARIMA} * 0.001 ,col sep=comma] {results/rpi4.csv}; \addlegendentry{ARIMA}

            \end{axis}
        \end{tikzpicture}
        }
    \subcaptionbox{Commodity Server (amd64)}
    {
        \begin{tikzpicture}
            \begin{axis}[
                xlabel={CPUs},
                ylabel={ms/sample},
                xmin=0, xmax=8,
                ymin=0, ymax=1400,
                xtick={0,1,2,3,4,5,6,7,8},
                ytick={0,200,400,600,800,1000,1200,1400},
                legend pos=north east,
                ymajorgrids=true,
                grid style=dashed,
            ]       
            \addplot table[x=cpu,y=CABIRCH,col sep=comma] {results/laptop.csv}; \addlegendentry{CABIRCH}
            \addplot table[x=cpu,y=LSTM,col sep=comma] {results/laptop.csv}; \addlegendentry{LSTM}
            \addplot table[x=cpu,y=ARIMA,col sep=comma] {results/laptop.csv}; \addlegendentry{ARIMA}
            \end{axis}
        \end{tikzpicture}
    }
    \caption{Experimental measurement of processing time per work item under varying resource limitations. Experiments with LSTM and ARIMA on RPI4 and other Raspberry models will follow.}
    \label{aa_experiments}
\end{figure*}


\section{Testbed}
The framework was deployed in a fog computing testbed depicted in Figure \ref{aiops_on_edge}. The infrastructure was divided in a cloud layer, representing a public or
private cloud and a fog layer describing the infrastructure between the cloud and the edge of the network.

\subsection{Cloud Layer}
In the cloud layer, the visualization stack consisting of InfluxDB and Grafana was deployed together with the decision engine. Since the Neo4j database we are
using for the dependency model has a high resource consumption and would therefore overload small edge device it was also deployed in the cloud layer.

In addition, the cloud layer also contains the IPFS Model storage which is synchronized with the the Model storages located in the fog layer. This enables the efficient exchange of models 
between the layers and further improves the reliability of the model storage.
\todo{describe how models are pinned inside of IPFS}
\todo{Event Bus broker}

Furthermore, resource-intensive data analysis steps like the anomaly analysis are scheduled in the cloud layer to relieve the edge devices.

\subsection{Fog Layer}
The fog layer consists out of the edge dewhilevices described in Table \ref{fog_devices} and represents an edge site in a fog computing infrastructure. 
The devices were categorized in two different types, gateway devices and edge devices.

\paragraph{Gateway devices}
Gateway devices are directly connected to the internet, i.e. via ethernet. As can be seen in Figure \ref{aiops_on_edge}, they create an ad-hoc mesh
network based on B.A.T.M.A.N-adv and serve as an internet gateway for the other mesh nodes in the infrastructure. The gateway devices act
as Kubernetes master nodes and edge devices can join the cluster using the mesh network connection.
In addition, a RabbitMQ cluster is deployed as a K8s StatefulSet across all gateway nodes to ensure availability of the event bus in case one of the nodes
breaks down.

\paragraph{Edge devices}
Edge devices are configured to join the mesh network using their Wifi interfaces. They register themselves as Kubernetes worker nodes at the gateway
devices via the mesh interface.

Sensors and actuators can be connected to the Raspberry Pi's GPIO pins, the USB ports, or via bluetooth. Running pods in the cluster directly access
the sensors using bind mounts in the container. One additional Wifi card is connected to one of the edge devices and configured to provide a  network which can be used
to administer the cluster.


Both device types run the data collection agent which is deployed as a DaemonSet across the Kubernetes cluster. The data collection agent gathers data from the
node including CPU, memory, network, I/O operation and pod metrics and provides the data as a data-stream. Furthermore, data-analysis steps like the anomaly-detection
are scheduled on the nodes. As the last component of the AIOps platform stack, every node runs the Model storage agent and uses it to store and exchange models
of analysis steps.

We further deployed an edge computing use case on the testbed to create realistic a realistic load scenario which is described in the next section.


\begin{figure*}[!h]
    \centering
    \includegraphics[width=1\textwidth]{images/AIOPS_EDGE.png}
    \caption{Fog computing testbed with placement of framework components.}
    \label{aiops_on_edge}
\end{figure*}


\begin{table}[h]
    \caption{Edge devices used in the testbed}
    \label{fog_devices}
    \footnotesize
    \begin{tabular}{|l|l|l|l|l|}
    \hline
    \rowcolor[HTML]{DAE8FC} 
    \# & Model                 & CPU                                                             & Memory & Network                                                                                       \\ \hline
    1  & Raspberry Pi 3B       & \begin{tabular}[c]{@{}l@{}}4× Cortex-A53\\ 1.2 GHz\end{tabular} & 1 GB   & \begin{tabular}[c]{@{}l@{}}100 Mbit/s\\ \\ 2.4 GHz Wifi\end{tabular}          \\ \hline
    2  & Raspberry Pi 3B+      & \begin{tabular}[c]{@{}l@{}}4× Cortex-A53\\ 1.4 GHz\end{tabular} & 1 GB   & \begin{tabular}[c]{@{}l@{}}1000 Mbit/s\\ \\  2.4/5 GHz Wifi\end{tabular}  \\ \hline
    2  & Raspberry Pi 4B (1GB) & \begin{tabular}[c]{@{}l@{}}4× Cortex-A72\\ 1.5 GHz\end{tabular} & 1 GB   & \begin{tabular}[c]{@{}l@{}}1000 Mbit/s \\ \\  2.4/5 GHz Wifi\end{tabular} \\ \hline
    1  & Raspberry Pi 4B (2GB) & \begin{tabular}[c]{@{}l@{}}4× Cortex-A72\\ 1.5 GHz\end{tabular} & 2 GB   & \begin{tabular}[c]{@{}l@{}}1000 Mbit/s\\ \\  2.4/5 GHz Wifi\end{tabular}  \\ \hline
    \end{tabular}
\end{table}


\subsection{Edge Computing Use Case}

\begin{itemize}
    \item Kafka + worker?
    \item smart city dataset
\end{itemize}

\subsection{Experiment setup}

\textbf{Model repository}

Retrieving of models:
\begin{itemize}
    \item deploy redis in cloud layer and store data in database / Store data in cloud IPFS node
    \item use several edge nodes to retrieve data from redis/IPFS
    \item measure network throughput on gateway node
    \item measure latency of requests
    \item plot network throughput and latency over time
    \item Assumption: network througput and latency will go down in case of IPFS, due to peer-to-peer transfers
\end{itemize}

==> 05-exp-results.tex <==
\section{Experimental results}
This section summarizes the evaluation. Main findings is the balance between used computational power and the precisions for anomaly detection. How much power do we have
to invest in order to achieve reasonable results without destroying the original IoT application running on the edge device?

